The Lean Data Scientist: Recent Advances towards Overcoming the Data Bottleneck

Machine learning (ML) is revolutionizing the world, affecting almost every field of science and industry. Recent algorithms (in particular, deep networks) are increasingly data-hungry, requiring large datasets for training. Thus, the dominant paradigm in ML today involves constructing large, task-specific datasets. However, obtaining quality datasets of such magnitude proves to be a difficult challenge. A variety of methods have been proposed to address this data bottleneck problem, but they are scattered across different areas, and it is hard for a practitioner to keep up with the latest developments. In this work, we propose a taxonomy of these methods. Our goal is twofold: (1) We wish to raise the community's awareness of the methods that already exist and encourage more efficient use of resources, and (2) we hope that such a taxonomy will contribute to our understanding of the problem, inspiring novel ideas and strategies to replace current annotation-heavy approaches.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.


==> data_programming.tex <==
\nnote{I do this part}

\begin{itemize}
    \item What is the problem
    \item How data programming solves the problem in general
    
    \item Different types of data-programming solutions, with many links
    
    \begin{itemize}
    
        \item \textbf{Snorkel}: \cite{ratner2019snorkel} Writing LPs, learn LP accuracies and correlations through clever (and super complex) generative model that is factor-graph based, use the accuracies and correlations to assign probabilistic label to each data point, use the probabilistic labels to train NN for final predictions (but this part is not related to the missing labels problem). Super popular, very intuitive, impressive results. Cited by 150.
        
        \item \textbf{Snuba, Babble Labble, Osprey}: All works that take Snorkel and improve it a bit. Usually making the LP generation easier.
        
        \item \textbf{Snuba} \cite{varma2018snuba}: Basically, they want to automatically find labeling functions. Couldn't find any code for this, so maybe just mention in one line in the Snorkel part. Actually don't find this very promising...
        
        \item \textbf{Babble Labble} \cite{hancock2018training}: Really cute concept, but I don't think it is very relevant to this paper -- it generates python functions from ``free'' text. You can let the turkers write LPs without knowing how to code! Cool! Will probably get in as a citation.
        
        \item \textbf{Osprey} \cite{bringer2019osprey}. Another work that takes Snorkel and improves it a bit.

    \end{itemize}
\end{itemize}

\nnote{working plan -- read each one of the articles above + some more. fill the bullets above. Simple}

% This category contains signals that are present in the data but

% based on known constraints regarding the proportions of labels in the different sub-groups that's in the data. 



==> sections/future_directions.tex <==
In the previous sections we introduced a taxonomy of ways to cope with the data bottleneck.
In addition to guiding researchers facing this bottleneck in their line of work, we hope the taxonomy could also help researchers develop new methods to tackle the problem. % highlight promising future research directions. 
In the following, we briefly demonstrate how the taxonomy could inspire future research directions -- either by integrating currently-disconnected methods (Section \ref{sec:future-integrate}) or by highlighting underlying assumptions (Section \ref{sec:future-assum}).
%suggest several such directions, inspired by the taxonomy.

\subsection{Integrating existing methods} 
\label{sec:future-integrate}
% \dnote{this is just a grocery list. what are the directions you actually think are promising?}

As noted earlier, many methods to tackle the data bottleneck are scattered across different areas. We now suggest several such disconnected methods that could nicely complement each other. 

\paragraph{\textbf{Wider meta-learning adoption}} Meta-learning trains general models that can later be fine-tuned to target tasks using little labeled data (Section \ref{sec:improve_model}). We posit meta-learning could be naturally combined with several other methods, especially transfer learning (Section \ref{sec:improve_model}) and self-supervision. Applying meta-learning in a pretraining step, for example, and then training using MAML \cite{maml}, may result in models that are easier to fine-tune later. 


% \dnote{I removed the following paragraph. Not clear if it has been studied from the text} \cnote{What do you mean? We even present an example to show the promise of this combination}

\paragraph{\textbf{Weak supervision \& multi-task learning}}
Weak signals usually refer to a subset of the examples for a single task; however, we believe that incorporating them into multi-task learning systems which can handle incomplete (e.g., \citep{Kokkinos2016UberNetTA}) labels and further improve the performance of these systems. 
Combining these approaches will make it possible to add even more diverse tasks to jointly optimize on, thus; will ease the burden of data collection.

For example, \citet{ratner2019training} incorporated weak signals on the multi-task dataset GLUE \cite{wang-etal-2018-glue}, where they achieved SOTA results.


\remove{
We believe another potential direction is integrating weak supervision (Section \ref{sec:relations}) with multi-task learning (Section \ref{sec:improve_model}). 

This approach was presented by \citet{ratner2019training}, where they achieved state-of-the-art results on the multi-task dataset GLUE \cite{wang-etal-2018-glue} by incorporating additional weak signals for multiple tasks into the training process. 
% For example, \citet{Kokkinos2016UberNetTA} presented UberNet, a multi-task based neural network that improves performance even if not all labels exist for each training example.
%

As weak signals usually refer to a subset of the examples for a single task \cite{ratner2019snorkel}, we believe that incorporating them into multi-task learning systems which can handle incomplete (e.g., \citep{Kokkinos2016UberNetTA}) labels will further improve the performance of these systems. 
Combining these approaches will make it possible to add even more diverse tasks to jointly optimize on, thus; will ease the burden of data collection.
}

\paragraph{\textbf{Feature importance \& marginal examples generation}} Marginal examples could be automatically generated based on the knowledge of features contributing the most. Currently, marginal examples generation does not explicitly use the different weights of features.
Without underestimating feature importance, we did not survey this method due to its simplicity. However, this powerful analysis tool can assist in creating examples that will be even more useful for the learner, potentially improving performance. % with the same or even fewer examples.
% \dnote{is it a combination of methods?} \cnote{Yes, using feature importance to better generate marginal examples.} \dnote{I mean, we didn't have feature importance in the taxonomy} \cnote{How about now? :)}

\subsection{Novel Directions}
\label{sec:future-assum}

The taxonomy makes it easy to identify underlying assumptions and highlight research questions that are currently not getting much attention\footnote{Including questions that do not get attention for good reasons.}. For example, what if we have an unrepresentative sample of data? What if we only have knowledge about the \emph{distributions} of both data points $P(\mathcal{X}=x)$ and labels $P(\mathcal{Y}=y)$, separately?  Below we suggest three such directions.

\paragraph{\textbf{Enhancing noisy labels}} An assumption that stands out due to the taxonomy is that each example has solely \emph{one correct label}. In practice, many labeling processes are based on crowdsourcing, and each data point often has many, possibly contradictory, labels created by multiple annotators. 
Instead of integrating the distribution of labels in the loss function \citep{Zhang2017mixupBE,hosseini2012aggregating}, or trying to find the most appropriate label \citep{zhao2012bayesian, kim2012bayesian, voorhees2000variations}, we offer to embrace the inter-annotators mismatch, just as a child learns from many, sometimes contradicting, sources (parents, teachers).
%
In practice, we suggest using the same example $x \in \mathcal{X}$, each time with a different $y \in \mathcal{Y}^*(x)$ (where $\mathcal{Y}^*(x)$ is the set of all labels annotated for $x \in \mathcal{X}$). 

We build upon the finding that noisy learning environments create models that are more robust to noise; however, they are usually created by adding random Bernoulli class-flip noise \citep{natarajan2013learning, liu2015classification, sukhbaatar2014training}. Instead, we offer to integrate human-generated noise, which is embedded in the task itself, rather than meaningless noise.

\remove{
In addition, using a majority vote to choose a label does not capture potential ambiguities of data points. 
For example, in humor detection tasks \cite{shahaf2015inside, taylor2004computationally, davidov2010semi, reyes2012humor, ptavcek2014sarcasm, bertero2016long} it is often the case where annotators' disagreement reflects the real ambiguity present in a data point, while ``forcing'' a binary label might be an unjustified over simplification. 
}

\paragraph{\textbf{Experts' local knowledge: argumentation-based machine learning (ABML)}} \dnote{is it related to Jerry's explanation-based learning?}

A direction we believe should get more attention is the use of \emph{experts' local knowledge} to constrain the search space \citep{clark1989cn2, movzina2007argument, rahwan2009argumentation, modgil2013added}. 
In a nutshell, in ABML the learner attempts to find if-then rules to explain argumented examples in a rule induction process. 
The learner starts by finding a rule, adding it to a set of rules and removing all training data points that are covered by that rule. This process is repeated until all examples are removed. 
ABML's main advantage is the use of expert knowledge to justify \emph{specific} examples, which is often easier than explaining global phenomena.

%However, it is rarely used due to the absent of expert knowledge and reasoning from mainstream datasets. Nevertheless, in the presence of such local knowledge, ABML is a powerful way to integrate partial prior knowledge for data-efficiently. Moreover, the induced hypothesis should make more sense to an expert, as it must be consistent with given arguments. 

For example, an application for ABML was developed by \citet{movzina2007argument}, who used medical records of deceased patients. They used a physician’s reasoning for the cause of death to limit the search space. 

\remove{
\paragraph{\textbf{Task specific self-supervision}}

Another direction that is not currently covered is the use of \emph{self-supervision} in a task-specific manner, rather than its standard embedding directed use (presented under transfer learning, see Section \ref{sec:improve_model}). 

\dnote{not clear what you mean by task-specific use. maybe an example?}
\cnote{I just realized that's how image reconstruction is done so can't really say that it's not used in vision. As for NLP, maybe can be used for tasks such as grammar error correction, but I'm not sure it hasn't been done already. Maybe we should drop this whole paragraph?} \dnote{if you're not sure it's new, then yes, drop it}

In self-supervised learning, the learner attempts to predict part of the input from other parts of it, i.e., a portion of the input is used as a supervisory signal while the remaining portion serves as input. This method is used to train on an unlabeled dataset in a supervised manner; the learner attempts to complete masked parts of the input from different parts of the very same input. This method's essence is that given one part of the object as input, the goal is to predict or generate the other part.

Although self-supervision is commonly used for finding an acceptable data representation, we argue in favor of a more task-specific use, towards solving the data bottleneck.

\citet{asano2019critical} recently emphasized the potential of this method in the context of data-efficiency. They showed that when using self-supervision and data augmentation, as little as a \emph{single image} is sufficient to learn the first few layers of standard deep networks, similar to using millions labeled images. Thus, it is possible to use a single image to learn the first few layers of a deep network almost ``perfectly.'' Regarding the deeper layers, they found that training these layers with self-supervision and a single image already achieves as much as two-thirds of the performance that can be achieved by using million different images.
Thus, we believe self-supervision should be more widely used in a task-specific manner.
}
